A constrained control-planning strategy for redundant manipulators

This paper presents an interconnected control-planning strategy for redundant manipulators, subject to system and environmental constraints. The method incorporates low-level control characteristics and high-level planning components into a robust strategy for manipulators acting in complex environments, subject to joint limits. This strategy is formulated using an adaptive control rule, the estimated dynamic model of the robotic system and the nullspace of the linearized constraints. A path is generated that takes into account the capabilities of the platform. The proposed method is computationally efficient, enabling its implementation on a real multi-body robotic system. Through experimental results with a 7 DOF manipulator, we demonstrate the performance of the method in real-world scenarios.

==> sections/proposed_method.tex <==
\tikzstyle{block} = [draw, fill=white, rectangle, 
    minimum height=3em, minimum width=6em]
\tikzstyle{sum} = [draw, fill=white, circle, node distance=1cm]
\tikzstyle{input} = [coordinate]
\tikzstyle{output} = [coordinate]
\tikzstyle{pinstyle} = [pin edge={to-,thin,black}]

\begin{figure*}
    \centering
    \begin{tikzpicture}[auto, node distance=2cm]
    
    \node [input, name=input] {};
    \node [block, right of=input, node distance=3cm] (ik){IK};
    \node [block, right of=ik, node distance=3cm] (ctrl){Controller};
    \node [block, right of=ctrl, node distance=3cm] (dyn){Dynamics};
    \node [block, right of=dyn,node distance=4cm] (opt){Optimization};
    \node [block, right of=opt,node distance=3cm] (robot){Robot};
    \node [output, right of=opt] (output) {};
    \node [output, below of=ik, node distance=1cm] (output_dyn2) {};
    \node [output, above of=robot, node distance=1cm] (output_dyn3) {};
     \node [output, above of=ctrl, node distance=1cm] (output_dyn4) {};
    \draw [draw,->] (input) -- node {$ee_{goal}$} (ik);
    \draw [->] (ik) -- node {$x_{goal}$} (ctrl);
    \draw [->] (ctrl) -- node {$\tau_i$} (dyn);
    \draw [->] (dyn) -- node {$x_{(i+1),des}$} (opt);
    \draw [->] (opt) -- node [name=des_input] {$u_i$}(robot);
    \draw [-] (robot) |- node[near end]  {$x_i$}(output_dyn2);
    \draw [->] (output_dyn2) |- node {}(ik.south);
    \draw [-] (ctrl) |- node  {}(output_dyn4);
    \draw [-] (output_dyn4) |- node[near end]  {$\tau_i$}(output_dyn3);
    \draw [->] (output_dyn3) -- node {}(robot);
    \end{tikzpicture}
    \caption{\small{The full pipeline of the proposed strategy: the \textbf{IK} component maps the desired end-effector goal to desired joint coordinates; \textbf{Controller} computes the low-level control forces and sends the commands to the robot and to the \textbf{Dynamics} component that estimates an initial path for the robot as described in Section~\ref{sub:lla_control}; the \textbf{Optimization} block (Section~\ref{sub:optimal}) incorporates the environmental constraints and produces the final path request and sends it to the \textbf{Robot}.}\vspace{-10pt}}
    \label{fig:pipeline}
\end{figure*}
%
%
%
In this section we present a path generation algorithm for redundant manipulation systems. A new method for generating a robust initial path estimation is described in  Section~\ref{sub:lla_control} and in Section \ref{sub:optimal} we incorporate this initial estimate together with inequality constraints into a prioritized-optimal control strategy.
The full pipeline of the proposed strategy can be seen in Figure~\ref{fig:pipeline}.

\vspace{-10pt}
\subsection{Adaptive path estimation}
\label{sub:lla_control}

We propose a strategy for defining a robust initial guess for optimal control strategies, that can be divided into two stages: $(a)$ design of a low-level control law and $(b)$ estimation of the initial path. 
%
%
\paragraph{Low-level control law}
In the first step the low-level control forces are computed using a strategy that requires one single parameter to be tuned and ensures robust behavior in the presence of system uncertainties. 
The controller has a feedback structure and has the capability to provide a reliable transient response. 
It is characterized by a single control loop for position control, Equation~\eqref{eq:feed_forward_adaptive_pid}, defined by the joint error, ${e_{x_i} = x_{goal}  - x_i}$.
The position goal, $x_{goal} \in \mathbb{R}^n$, represents the final joints desired configuration.
Using an iterative formulation the feedback control law, with gravity compensation, is defined as:
\begin{equation}
    \tau_i =  \gamma \Lambda(e_{{x}_i}) + \eta
    \label{eq:feed_forward_adaptive_pid}
\end{equation}
where $\gamma \in \mathbb{R}^n$ is the adaptive gain parameter that describes the rate of change of the controller, $\tau_i \in \mathbb{R}^n$ is the control input for all the joints of the manipulator, at time-step $i$ and $\Lambda$ is a nonlinear function dependent on the joint errors defined:  
\vspace{-10pt}
\begin{equation}
\begin{aligned}
\Lambda(e_{{x}_i}) =  e_{{x}_i}^3 + e_{{x}_i} \left( \frac{e_{{x}_i} - e_{{x}_{i-1}}}{\Delta t}\right) ^2  +  e_{{x}_i}  \left( \sum_{j=0}^i  e_{{x}_j} \Delta t \right)^2 
\end{aligned}
    \label{eq:control_function}
\end{equation}
%
Similar to a \ac{PID} controller Equation~(\ref{eq:control_function}) aims to eliminate residual error and estimate the future behaviour of the system. 
By using a formulation that is proportional, and of equal sign to the change in the control error, the proposed  method is able to drive the system to steady-state. 
Furthermore, it is only dependent on a single parameter that characterizes the rate of change in the controller. 

\paragraph{Path estimation}
In this stage we use the low-level control law defined in the previous step with an estimated dynamic model to generate the initial path estimation.
\begin{equation}
\begin{aligned}
\hat{x}_{(i+1), {des}} = & Ax_i +B\tau_i \\
\hat{u}_{i, {des}} = & Gx_i
\end{aligned}
\label{eq:estimated_path}
\end{equation}
where $x_{(i+1), {des}} \in \mathbb{R}^n$ represents the initial estimate path, $A \in \mathbb{R}^{n \times n}$, $B \in \mathbb{R}^{n \times m}$, $G \in \mathbb{R}^{m \times n}$ represent the estimated system, input and output matrices obtained from the dynamic model of the platform. Due to uncertainties in the mathematical model of the robot these values are approximated.

\vspace{-10pt}
\subsection{Optimal-Adaptive path generation}
\label{sub:optimal}
The estimated path defined in Equation~(\ref{eq:estimated_path}) takes into account the torque limitations but does not incorporate environmental constraints or the physical limitations of the system. 
To address these we use a null-space constrained optimal formulation, Equation~(\ref{eq:problem_statement}), to obtain solutions for a feasible path. 
This approach has been used for prioritized-optimal control previously in \cite{de2009prioritized} and \cite{romano2015prioritized} for low-level control structures. 
We extend the work presented in \cite{giftthaler2017projection} by proposing a solution that handles inequality constraints. 
%
 \subsubsection{Inequality constraints}

In this section we introduce the inequality constraints to the control problem.
We use the artificial potential field approach as an effective real-time method for incorporating constraints. 
This approach has been demonstrated for state and state-input constraints such as joint limits and obstacle avoidance \cite{khatib1986real}.
 
State constraints can be expressed as Equation (\ref{eq:joint_limits_min}), if a \textit{minimum} problem is described, or as Equation (\ref{eq:joint_limits_max}) for a \textit{maximum} problem:
\begin{equation}
    h_2(x_i, i) = \begin{cases}
     \eta \left( \frac{1}{\underline{\rho}_i} - \frac{1}{\underline{\rho}_0} \right) \frac{1}{\underline{\rho}_i^2}, & \quad \text{if $\underline{\rho}_i \leq \underline{\rho}_0$}    \\ \!
      0, & \quad \text{if $\underline{\rho}_i > \underline{\rho}_0$}
    \end{cases}
    \label{eq:joint_limits_min}
\end{equation}
%
\vspace{-30pt}
\begin{equation}
    h_3(x_i, i) = \begin{cases}
     - \eta \left( \frac{1}{\bar{\rho}_i} - \frac{1}{\bar{\rho}_0} \right) \frac{1}{\bar{\rho}_i^2}, & \quad \text{if $\bar{\rho}_i \leq \bar{\rho}_0$}    \\ \!
      0, & \quad \text{if $\bar{\rho}_i > \bar{\rho}_0$}
    \end{cases}
    \label{eq:joint_limits_max}
\end{equation}

where $\underline{\rho}_0$ and $\bar{\rho}_0$ represent the distance limit to the potential field, $\underline{\rho}_i = x_i - \underline{x}_i$ is the distance from the minimum limit, and $\bar{\rho}_i = \bar{x}_i - x_i$ is the distance from the maximum limit. As presented by \citet{khatib1986potential} this method of representing system limitations and obstacle avoidance is an attractive approach, as it provides the global information necessary for robot control applications. 



\subsubsection{Optimal framework formulation}
Following work done in \cite{li2004iterative}, \cite{murray1984differential} and \cite{del2014prioritized}, the Newton's method for nonlinear minimization is used to reformulate the optimal formulation presented in Equation (\ref{eq:problem_statement}). 
%Starting from an initial solution, linear approximations of the current dynamic model, cost function and priority constraints are defined
A new linear-quadratic constrained problem that describes the effects of perturbations on the state variables (joint positions) and input variables (joint velocities) is defined, allowing an iterative formulation of the initial optimization problem. The displacement from the measured state, $\Delta x_i = x_i - \hat{x}_{i,{des}}$ and from the input state $\Delta u_i = u_i - \hat{u}_{i,{des}}$ are expressed based on the estimated desired joint positions and velocities in Equation~(\ref{eq:estimated_path}).

Using these displacements, the inequality constraints presented in Equations~(\ref{eq:joint_limits_min})-(\ref{eq:joint_limits_max}), the optimal control problem expressed by Equations~ (\ref{eq:problem_statement})-(\ref{eq:constraint_2}) can now be reformulated dependent on the state and input deviations as a linear quadratic control problem:
 \begin{equation}
 \begin{aligned}
    \Delta u^{*}_i =  \min_{\Delta u_i} &\lbrace  o_N + \Delta x_N^T q_N + \frac{1}{2} \Delta x_N^T Q_N + \Delta x_N  + \\ \!
    & + \sum_{i=0}^{N-1} o_i + \Delta x_i q_i + \Delta u_i^T r_i + \frac{1}{2} \Delta x_i^T Q_i \Delta x_i +  \\ \!
    & + \frac{1}{2} \Delta u_i^T R_i \Delta u_i + \Delta u_i^T P_i \Delta x_i  \rbrace
\end{aligned}
      \label{eq:problem_statement_final}
  \end{equation}
  subject to:
 \begin{equation}
    \Delta x_{i+1} = A_i \Delta x_i + B_i \Delta u_i, \quad x(0) =x_0
    \label{eq:dynamic_eq_final}
\end{equation}
\begin{equation}
    D_i \Delta x_i  = e_i %+ E_i \Delta u_i
    \label{eq:constraint_1_final}
\end{equation}
\begin{equation}
    C_i \Delta x_i = d_i
    \label{eq:constraint_2_final}
\end{equation}

where $o, \ q, \ r, \ Q, \ R, \ P $ are coefficients of the Taylor expansion of Equation (\ref{eq:problem_statement}) around the estimated states. 
The linearized dynamics are presented in Equation (\ref{eq:dynamic_eq_final}) and the inequality constraints are re-defined using the potential fields in  Equations (\ref{eq:constraint_1_final}) - (\ref{eq:constraint_2_final}). To handle any possible discontinuities in the formulation of the constraints we used the method presented in \cite{stella2016very}.
%
The goal is to solve this local-optimal control law generating a planning policy update, $\Delta u_i(x_i)$, which will be used in the global formulation:
\begin{equation}
    u_i(x_i) = u_i(x_i) + \Delta u_i(x_i)
    \label{eq:final_ctrl_law}
\end{equation}
This planning policy update is responsible in refining the initial planning strategy defined by Equation~(\ref{eq:estimated_path}), taking into account restrictions caused by the working environment and generating an optimal trajectory.  

Following the work of \citet{giftthaler2017projection}, we use the nullspace projection theory to present a solution for the optimal formulation in Equation (\ref{eq:problem_statement_final}), by:
\begin{equation}
   \Delta u_i = \Delta u_i^c + \mathcal{N}\left( \begin{bmatrix}
    E_i\\
    M_i
    \end{bmatrix} \right) \Delta u_i^m
    \label{eq:null_space_reform}
\end{equation}
where $\Delta u_i^c$ is the constrained  control component that ensures the constraints are always fulfilled, $E_i = D_{i+1}B_i$ and $M_i = C_{i+1} B_i$ are the propagation of the input displacements to the next step of the constraints and $\mathcal{N}$ is the projection of the nullspace of these linearized constraints. $\Delta u_i^m$ is the control component that will ensure a valid solution to the optimal problem without breaking the constraints.

The constrained control law, $\Delta u_{i}^c$, is defined to satisfy the dynamics of the constraints at the next step in time. To achieve this we propose the use of feedforward-feedback strategy:
\begin{equation}
     \Delta u_{i}^c =  \begin{bmatrix}
    E_i\\
    M_i
    \end{bmatrix}^{\dagger} 
      \begin{bmatrix}
    e_{i+1}\\
    d_{i+1}
    \end{bmatrix} -  \begin{bmatrix}
    E_i\\
    M_i
    \end{bmatrix}^{\dagger}  \begin{bmatrix}
    F_i\\
    N_i
    \end{bmatrix} (\Delta x_{i_{des}} + \alpha)
    \label{eq:feed_forward}
\end{equation}
where $ \left[ E_i^T, \ M_i^T \right]^{\dagger} $ is the unweighted Moore-Penrose pseudoinverse matrix. $F_i = D_{i+1}B_i$ and $N_i = C_{i+1}B_i$ are the propagation of the state displacements to the next step of the constraints. To compensate for the disturbances in the actuators and inaccuracies in the robot unmodeled dynamics (damping and friction), we propose to introduce a feedback law, $\alpha \in \mathbb{R}^6$,  to make the control scheme robust. The proposed feedback law is of the same type as the one presented in Section \ref{sub:lla_control}, in this case being directly dependent of the difference between the estimated state, $x_{i_{des}}$ and the measured joint positions, $x_i$. 



\begin{figure*}[!htb]
    \centering
    \begin{subfigure}[b]{0.30\textwidth}
        \includegraphics[trim=10 0 30 0,clip,width=\textwidth]{figures/ee_x_lqr.png}
        \caption{X end-effector position}
        \label{fig:x_pos}
    \end{subfigure}
    ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
      %(or a blank line to force the subfigure onto a new line)
    \begin{subfigure}[b]{0.30\textwidth}
        \includegraphics[trim=10 10 10 10,clip,width=\textwidth]{figures/ee_y_lqr.png}
        \caption{Y end-effector position}
        \label{fig:y_pos}
    \end{subfigure}
    ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
    %(or a blank line to force the subfigure onto a new line)
    \begin{subfigure}[b]{0.30\textwidth}
        \includegraphics[trim=10 10 10 0,clip,width=\textwidth]{figures/ee_z_lqr.png}
        \caption{Z end-effector position}
        \label{fig:z_pos}
    \end{subfigure}
    \caption{\small{Comparison of end-effector behavior using Optimal-Adaptive method, Optimal-LQR method, Adaptive strategy, \ac{RRT} and \ac{EST} methods to reach a discrete point defined in world coordinates at $(0.81, -0.05, 0.8)$ meters.  The \ac{RRT} and \ac{EST} methods require more than $4$ seconds to compute a plan but have a very fast execution, while for the Adapt and Optimal-Adapt methods the execution  starts as soon as the first waypoint is generated, leading to a slower but more gradual movement. Using the Optimal-LQR method presents a higher variation from the set-point, showcasing the limitation of an inaccurate initial guess.}}\label{fig:ee_x_y_z}
\end{figure*}
%
%
\begin{figure*}[!htb]
  \centering
    \begin{subfigure}[]{\columnwidth}
    \centering
     \includegraphics[width=0.75\columnwidth]{figures/joint_error_adapt_v2.png}
     \caption{Adaptive joint errors}
     \label{fig:error_adapt}
     \end{subfigure}
 \begin{subfigure}[]{\columnwidth}
    \centering
     \includegraphics[width=0.75\columnwidth]{figures/joint_error_optimal_v2.png}
     \caption{Optimal-Adaptive joint errors}
     \label{fig:error_optim}
     \end{subfigure}
     \caption{\small{Joint angle errors for the (a) initial Adaptive strategy and the (b) Optimal-Adaptive method when the end-effector behaviour is the one presented in Figure~\ref{fig:ee_x_y_z}. The Optimal-Adaptive strategy reduces significantly the time needed for the joints to reach the desired configuration compared with the initial Adaptive strategy, where also Joint $5$ is not able to reach the desired configuration, leading to an offset from the goal.}}
     \label{fig:joint_traj}
\end{figure*}
%
%
 %
Incorporating Equations~(\ref{eq:null_space_reform})-(\ref{eq:feed_forward}) into the optimal formulation expressed by Equation (\ref{eq:problem_statement_final}), the optimal path that does not violate the constraints of the problem is defined as the solution of:
%
\begin{equation}
 \begin{aligned}
    \Delta u^{m*}_i =  \min_{\Delta u_i^m} &\lbrace  o_N + \Delta x_N^T q_N + \frac{1}{2} \Delta x_N^T Q_N + \Delta x_N  + \\
    & + \sum_{i=0}^{N-1} \tilde{o}_i + \Delta x_i \tilde{q}_i + \Delta {u_i^m}^T \tilde{r}_i + \frac{1}{2} \Delta x_i^T \tilde{Q}_i \Delta x_i +  \\
    & + \frac{1}{2} \Delta {u_i^m}^T \tilde{R}_i \Delta u_i^m + \Delta {u_i^m}^T \tilde{P}_i \Delta x_i  \rbrace
\end{aligned}
      \label{eq:problem_statement_reformulated_u}
  \end{equation}
  subject to
  \begin{equation}
    \Delta x_{i+1} = \tilde{A}_i \Delta x_i + \tilde{B}_i \Delta u_i^m + \tilde{k}_i, \quad x(0) =x_0
    \label{eq:dynamic_eq_reformulated_u}
\end{equation}
where
\begin{equation}
    \begin{aligned}
   \tilde{A}_i & = A_i + B_i \Gamma_i  \\
    %
    \!
    \tilde{B}_i & = B_i \mathcal{N(\cdot)} \\
    %
    \!
    \tilde{g}_i & = B_i \Theta_i \\
    %
    \!
    \tilde{o}_i & = o_i +  \Theta_i^T r_i + \frac{1}{2} \Theta_i^T R_i \Theta_i \\
    %
    \!
    \tilde{q}_i & = q_i + \Gamma^T r_i + P_i^T \Theta_i + \Gamma_i^TR_i \Theta_i \\
    %
    \!
    \tilde{r} & = \mathcal{N}(\cdot) \left(r_i + R_i \Gamma_i \right) \\
    %
    \!
    \tilde{Q}_i & = Q_i + \Gamma_i^T R_i \Gamma_i + \Gamma_i^T P_i + P_i^T \Gamma_i \\
    %
    \!
    \tilde{R}_i & = \mathcal{N}(\cdot) R_i \mathcal{N}(\cdot) \\
    %
    \!
    \tilde{P}_i & = \mathcal{N}(\cdot) \left(P_i + R_i \Gamma_i \right)
    \end{aligned}
    \label{eq:reparametrization}
\end{equation}

The solution of this optimal structure is computed using a Riccati equation formulation \cite{kuvcera1972discrete}, producing a feedback law presented in Equation (\ref{eq:optimal_ctrl_output}). 
\begin{equation}
\begin{aligned}
     \Delta u_i^m & = -\left( \tilde{R}_i + \tilde{B}_i^TS_{i+1}\tilde{B}_i\right)^{\dagger} \lbrace (\tilde{P}_i + \tilde{B}_i^TS_{i+1}\tilde{A}_i) \Delta x_i - \\
     & -\left[\tilde{r}_i + \tilde{B}_i^T(s_{i+1}+S_{i+1} k_i)\right] \rbrace
\end{aligned}
    \label{eq:optimal_ctrl_output}
\end{equation}
where $S_{i+1} \in \mathbb{R}^{n \times n}$ and $s_{i+1} \in \mathbb{R}^{n}$ are weighting matrices. 

The computational cost of the final planning solution, Equation (\ref{eq:final_ctrl_solution}), allows for  real-time implementation of this strategy on high-dimensional robotic systems, ensures the constraints of the problem are fulfilled and generates plans that can be fulfilled by the low-level controller. 
\begin{equation}
    \hat{u}_{i} = \hat{u}_{i_{des}} + \Delta u_i^c + \mathcal{N}(\cdot) \Delta u_i^m
    \label{eq:final_ctrl_solution}
\end{equation}

\begin{figure*}[!htb]
  \centering
    \begin{subfigure}[]{0.30\textwidth}
        \includegraphics[trim=10 0 10 0,clip, width=\textwidth]{figures/error_ee_x_lqr.png}
         \caption{Error in X}
         \label{fig:err_x_lqr}
     \end{subfigure}
     ~
    \begin{subfigure}[]{0.30\textwidth}
        \includegraphics[trim=10 0 10 0,clip, width=\textwidth]{figures/error_ee_y_lqr.png}
        \caption{Error in Y}
        \label{fig:err_y_lqr}
    \end{subfigure}
    ~
    \begin{subfigure}[]{0.30\textwidth}
        \includegraphics[trim=10 0 10 0,clip, width=\textwidth]{figures/error_ee_z_lqr.png}
        \caption{Error in Z}
        \label{fig:err_z_lqr}
    \end{subfigure}
    \caption{\small{End-effector error for the case when the joint limit presented in Figure~\ref{fig:joint_restricted} is imposed: the Optimal-Adapt (proposed) strategy reaches the vicinity of the goal fulfilling the constraints while the Optimal-LQR has a higher end-effector error, highlighting the importance of a reliable initial estimate. The \ac{RRT} method presents better accuracy  compared with any other method, nevertheless the constraints are broken and the \ac{EST} breaks the limits and also has a worse end-effector error.}\vspace{-10pt}}
     \label{fig:errors_ee}
\end{figure*}
%
\begin{figure}[!htb]
  \centering
    \includegraphics[width=0.75\columnwidth]{figures/joint1_limit_lqr.png}
     \caption{\small{Behaviour of Joint $1$ for the case when it can move only between ($-0.1$, $0.1$) radians. The proposed Optimal-Adapt strategy succeeds in maintaining the joint between the boundaries (in the shaded area of the graph) as well as the Optimal-LQR method, as they both rely on the same priority-optimal principle that handles constraints.}\vspace{-10pt}}
     \label{fig:joint_restricted}
\end{figure}





==> sections/proposed_method__Matthew_Johnson-Roberson_s_conflicted_copy_2018-09-17_.tex <==
\tikzstyle{block} = [draw, fill=white, rectangle, 
    minimum height=3em, minimum width=6em]
\tikzstyle{sum} = [draw, fill=white, circle, node distance=1cm]
\tikzstyle{input} = [coordinate]
\tikzstyle{output} = [coordinate]
\tikzstyle{pinstyle} = [pin edge={to-,thin,black}]

\begin{figure*}
    \centering
    \begin{tikzpicture}[auto, node distance=2cm]
    % We start by placing the blocks
    \node [input, name=input] {};
    \node [block, right of=input, node distance=3cm] (ik){IK};
    \node [block, right of=ik, node distance=3cm] (ctrl){Controller};
    \node [block, right of=ctrl, node distance=3cm] (dyn){Dynamics};
    \node [block, right of=dyn,node distance=4cm] (opt){Optimization};
    \node [block, right of=opt,node distance=3cm] (robot){Robot};
    % \node [sum, right of=input] (sum_p) {};
    % \node [block, right of=sum_p] (controller_p){Position  Control};
    % \node [sum, right of=controller_p, node distance=2cm] (sum_v) {};
    % \node [block, right of=sum_v] (controller_v){Velocity Control};
    % \node [block, right of=controller_v, node distance=4cm] (auv){AUV};
    % \node [block, below of=auv, node distance=1.2cm] (dynamics){Dynamics};
    \node [output, right of=opt] (output) {};
    % \node [output, right of=output, node distance=0.4cm] (ooutput) {};
    % \node [output, right of=dynamics, node distance=1.4cm] (output_dyn) {};
    % \node [output, right of=output_dyn, node distance=1cm] (ooutput_dyn) {};
    \node [output, below of=ik, node distance=1cm] (output_dyn2) {};
    \node [output, above of=robot, node distance=1cm] (output_dyn3) {};
     \node [output, above of=ctrl, node distance=1cm] (output_dyn4) {};
    % \node [output, below of=output_dyn, node distance=1.1cm] (output_dyn3) {};
    % \node [block, right of=controller, pin={[pinstyle]above:Disturbances},
    %         node distance=3cm] (system) {System};
    % We draw an edge between the controller and system block to 
    % calculate the coordinate u. We need it to place the measurement block. 
    % \node [output, right of=system] (output) {};
    % \node [block, below of=u] (measurements) {Measurements};
    % % Once the nodes are placed, connecting them is easy. 
    \draw [draw,->] (input) -- node {$ee_{goal}$} (ik);
    \draw [->] (ik) -- node {$x_{goal}$} (ctrl);
    \draw [->] (ctrl) -- node {$\tau_i$} (dyn);
    \draw [->] (dyn) -- node {$x_{(i+1),des}$} (opt);
    \draw [->] (opt) -- node [name=des_input] {$u_i$}(robot);
    \draw [-] (robot) |- node[near end]  {$x_i$}(output_dyn2);
    \draw [->] (output_dyn2) |- node {}(ik.south);
    \draw [-] (ctrl) |- node  {}(output_dyn4);
    \draw [-] (output_dyn4) |- node[near end]  {$\tau_i$}(output_dyn3);
    \draw [->] (output_dyn3) -- node {}(robot);
    
    % \draw [->] (dynamics) -- node [name=w, near start] {$w$}(ooutput_dyn);
    % \draw [->] (controller_v) -- node[name=tau] {$\tau_Z$} (auv);
    %  \draw [->] (tau) |- node[near end] {} (dynamics);
    % \draw [-] (output_dyn) -|  (output_dyn2);
    % \draw [->] (output_dyn2) -| (sum_v);
    % \draw [-] (output) |-  (output_dyn3);
    % \draw [->] (output_dyn3) -| (sum_p);
    % \draw [->] (z) |- (sum_p);
    % \draw [->] (y) |- (measurements);
    %\draw [->] (output_dyn.south) |- node[pos=0.1] {$-$} node [near end] {$w$} (sum_v.south);
    \end{tikzpicture}
    \caption{\small{The full pipeline of the proposed strategy: the \textbf{IK} component maps the desired end-effector goal to desired joint coordinates; \textbf{Controller} computes the low-level control forces as described in Section~\ref{sub:lla_control} and sends the commands to the robot and to the \textbf{Dynamics} component that estimates an initial path for the robot (Section~\ref{sub:optimal}); the \textbf{Optimization} block incorporates the environmental constraints and produces the final path request and sends it to the \textbf{Robot}.}}
    \label{fig:pipeline}
\end{figure*}
%
%
In this section we present a path generation algorithm for redundant manipulation systems. A new method for generating a robust initial path estimation is described in  Section~\ref{sub:lla_control} and in Section \ref{sub:optimal} we incorporate this initial estimate together with inequality constraints into a prioritized-optimal control strategy.
The full pipeline of the proposed strategy can be seen in Figure~\ref{fig:pipeline}.
%
%
%We propose an algorithm for obtaining an optimal path for robotic manipulators based on three components: \textit{(i)} a feedback low-level control law; \textit{(ii)} initial estimation of manipulator path using the control law from the previous point and the dynamic model of the system; and \textit{(iii)} generation of a feasible path from the initial generated path based on a prioritized optimal formulation. 
%In Section~\ref{sub:lla_control} we present the low-level control structure together with the initial estimated path for the manipulator, followed by a description of the optimization strategy used to achieve a feasible path in Section~\ref{sub:optimal}. 
%\Ram{I am still confused as to what exactly you are doing. Maybe an algorithm box would help?}
\vspace{-10pt}
\subsection{Adaptive path estimation}
\label{sub:lla_control}
%Optimal control and planning solutions rely on an initial guess which has an important influence on the final result \cite{rieck2014generation}. 
% We propose a new method for generating a robust initial solution estimate that is directly dependent on the low-level control forces and an estimated dynamic model. For this stage we base the methodology on the general dynamic model describing a robotic manipulator, described at each time step as:
% \begin{equation}
%     M(\theta_i) \ddot{\theta_i} + C(\theta_i, \dot{\theta}_i) \dot{\theta}_i + \eta = \tau_i
%     \label{eq:dynamic_model}
% \end{equation}
% where the joint positions are represented by $\theta_i \in \mathbb{R}^n$, the inertia matrix is $M(\theta_i) \in \mathbb{R}^{n \times n}$, $C(\theta_i, \dot{\theta}_i) \in \mathbb{R}^{n}$ is the Coriolis vector, and $\eta \in \mathbb{R}^n$ represents the gravity force. 
%
We propose a strategy for defining a robust initial guess for optimal control strategies, that can be divided into two stages: $(a)$ design of a low-level control law and $(b)$ estimation of the initial path. 
%
%
\paragraph{Low-level control law}
In the first step the low-level control forces are computed using a strategy that requires one single parameter to be tuned and ensures robust behavior in the presence of system uncertainties. 
The controller has a feedback structure and has the capability to provide a reliable transient response. 
It is characterized by a single control loop for position control, Equation~\eqref{eq:feed_forward_adaptive_pid}, defined by the joint error, ${e_{x_i} = x_{goal}  - x_i}$.
The position goal, $x_{goal} \in \mathbb{R}^n$, represents the final joints desired configuration.
Using an iterative formulation the feedback control law, with gravity compensation, is defined as:
\begin{equation}
    \tau_i =  \gamma \Lambda(e_{{x}_i}) + \eta
    \label{eq:feed_forward_adaptive_pid}
\end{equation}
where $\gamma \in \mathbb{R}^n$ is the adaptive gain parameter that describes the rate of change of the controller, $\tau_i \in \mathbb{R}^n$ is the control input for all the joints of the manipulator, at time-step $i$ and $\Lambda$ is a nonlinear function dependent on the joint errors defined by:  
\vspace{-10pt}
\begin{equation}
\begin{aligned}
\Lambda(e_{{x}_i}) =  e_{{x}_i}^3 + e_{{x}_i} \left( \frac{e_{{x}_i} - e_{{x}_{i-1}}}{\Delta t}\right) ^2  +  e_{{x}_i}  \left( \sum_{j=0}^i  e_{{x}_j} \Delta t \right)^2 
\end{aligned}
    \label{eq:control_function}
\end{equation}
%
Similar to a \ac{PID} controller Equation~(\ref{eq:control_function}) aims to eliminate residual error and estimate the future behaviour of the system. 
By using a formulation that is proportional and of equal sign to the change in the control error the proposed  method is able to drive the system to steady-state. 
Furthermore, it is only dependent on a single parameter that characterizes the rate of change in the controller. 
%This control law was chosen as it is directly dependent on the behaviour of the system, is not prone to oscillations, provides a robust response, and has a small convergence time \Ram{why are these properties true?}. 

\paragraph{Path estimation}
In this stage we use the low-level control law defined in the previous step with an estimated dynamic model to generate the initial path estimation.
\begin{equation}
% \begin{aligned}
%     \ddot{\theta}_{i,_{des}} = & \hat{M}^{\dagger}\left(\tau_i - \hat{C}(\theta_i)\dot{\theta_i} - \eta \right) \\
%     \hat{u}_{i,_{des}} = &  \hat{u}_{{(i-1)}_{des}} + \ddot{\theta}_{i_{des}} \Delta t \\
%     \hat{x}_{i_{des}} = & \hat{x}_{{(i-1)}_{des}} + \hat{u}_{i_{des}} \Delta t +  \ddot{\theta}_{i_{des}} \left( \Delta t \right)^2
% \end{aligned}
\begin{aligned}
\hat{x}_{(i+1), {des}} = & Ax_i +B\tau_i \\
\hat{u}_{i, {des}} = & Gx_i
\end{aligned}
\label{eq:estimated_path}
\end{equation}
where $x_{(i+1), {des}} \in \mathbb{R}^n$ represents the initial estimate path, $A \in \mathbb{R}^{n \times n}$, $B \in \mathbb{R}^{n \times m}$, $G \in \mathbb{R}^{m \times n}$ represent the estimated system, input and output matrices obtained from the dynamic model of the platform. Due to uncertainties in the mathematical model of the robot these values are approximated.
% \Ram{1.what is $\delta t$?2. What is the relationship between $x$ and $u$ in this problem and otpimal control problem you present in the problem formulation section 3. Its also strange because now you are using $\theta$ which i assumed was a part of your state in the optimal control problem formulation but it seems its distinct. 3. i'd recommend using a comma between different terms in the subscript}
%where $\ddot{\theta}_{i_{des}} \in \mathbb{R}^n$, $\hat{u}_{i_{des}}  \in \mathbb{R}^n$,  $\hat{x}_{i_{des}} \in \mathbb{R}^n$ are the estimated desired joint accelerations, velocities and positions computed at time-step $i$.  Due to uncertainties in the system an approximation of the pseudo-inverse of the inertia matrix, ${\hat{M}^{\dagger} \in \mathbb{R}^{n \times n}}$, and Coriolis vector, $\hat{C} \in \mathbb{R}^{n}$ are used. 

%The proposed strategy is characterized by the following behaviour: when the current state is far from the final goal, large forces \Ram{wnhat does large mean?} are generated leading to a fast planning response, but as the goal is significantly \Ram{what does significant mean?} closer, the planner generates way-points at smaller \Ram{smaller than?} interval, leading to a slower response \Ram{slower than?} from the system. 
%This leads to a very small \Ram{what is very small?} overshoot in the proximity of the goal, even in the presence of an approximated dynamic model \Ram{is this a proof or just an empirical observation?}.   


%Starting from this initial control output and the initial conditions  $x_0 \in \mathbb{R}^n$, in each iteration the estimated state $\hat{x}_i$ is computed using the dynamic equation, and the estimated control  input $\hat{u}_i$ is determined using the current control policy.
\vspace{-10pt}
\subsection{Optimal-Adaptive path generation}
\label{sub:optimal}
The estimated path defined in Equation~(\ref{eq:estimated_path}) takes into account the torque limitations but does not incorporate environmental constraints or the physical limitations of the system. 
To address these we use a null-space constrained optimal formulation, Equation~(\ref{eq:problem_statement}), to obtain solutions for a feasible path. 
This approach has been used for prioritized-optimal control previously in \cite{de2009prioritized} and \cite{romano2015prioritized} for low-level control structures. 
We extend the work presented in \cite{giftthaler2017projection} by proposing a solution that handles inequality constraints. 

 \subsubsection{Inequality constraints}
% As Equation (\ref{eq:constraint_1}) and Equation (\ref{eq:constraint_2}) define state constraints to the system, it is straightforward \Ram{what does straightforward mean?} to introduce these types of inequality constraints to the control problem.
In this section we introduce the inequality constraints to the control problem.
We use the artificial potential field approach as an effective real-time method for incorporating constraints. 
This approach has been demonstrated for state and state-input constraints such as joint limits and obstacle avoidance \cite{khatib1986real}.
% Assuming Equation (\ref{eq:constraint_1}) is defining an obstacle avoidance constraint using the potential field approach, this constraint is expressed by:
% \begin{equation}
%      h_1(x_i, u_i, i) = \begin{cases}
%      J^T \eta \left( \frac{1}{\rho_i} - \frac{1}{\rho_0}    \right) \frac{1}{\rho_i^2} \frac{\partial \rho_i}{ \partial p_i}, & \quad \text{if $\rho_i \leq \rho_0$} \\
%      0, & \quad \text{if $\rho > \rho_0$}
%      \end{cases}
%     \label{eq:obstacle_avoidance}
% \end{equation}
% where $\rho_0$ is the limit distance to the potential field, $\eta$ is a constant gain, $\rho_i$ is the shortest distance to the obstacle in end-effector coordinates, and $\frac{\partial \rho_i}{ \partial p_i}$ is the partial derivative of the distance with respect to the end-effector position ${p_i=\left[x_{ee}, \ y_{ee}, \ z_{ee} \right]^T}$. $J \in \mathbb{R}^{6 \times n}$ represents the transformation to the state representation.  
State constraints can be expressed as Equation (\ref{eq:joint_limits_min}), if a \textit{minimum} problem is described, or as Equation (\ref{eq:joint_limits_max}) for a \textit{maximum} problem:
\begin{equation}
    h_2(x_i, i) = \begin{cases}
     \eta \left( \frac{1}{\underline{\rho}_i} - \frac{1}{\underline{\rho}_0} \right) \frac{1}{\underline{\rho}_i^2}, & \quad \text{if $\underline{\rho}_i \leq \underline{\rho}_0$}    \\
      0, & \quad \text{if $\underline{\rho}_i > \underline{\rho}_0$}
    \end{cases}
    \label{eq:joint_limits_min}
\end{equation}
%
\vspace{-10pt}
\begin{equation}
    h_3(x_i, i) = \begin{cases}
     - \eta \left( \frac{1}{\bar{\rho}_i} - \frac{1}{\bar{\rho}_0} \right) \frac{1}{\bar{\rho}_i^2}, & \quad \text{if $\bar{\rho}_i \leq \bar{\rho}_0$}    \\
      0, & \quad \text{if $\bar{\rho}_i > \bar{\rho}_0$}
    \end{cases}
    \label{eq:joint_limits_max}
\end{equation}
%\Ram{1. Its not clear why this is capable of expressing obstacle avoidance and joint limit constraints. 2. This does not seem differentiable which makes applying optimization based techniques seem dangerous.}
where $\underline{\rho}_0$ and $\bar{\rho}_0$ represent the distance limit to the potential field, $\underline{\rho}_i = x_i - \underline{x}_i$ is the distance from the minimum limit, and $\bar{\rho}_i = \bar{x}_i - x_i$ is the distance from the maximum limit. As presented by \citet{khatib1986potential} this method of representing system limitations and obstacle avoidance is an attractive approach, as it provides the global information necessary for robot control applications. 

%The problem can be reformulated into a more restrictive formulations by:

%  \begin{equation}
%     u^{*}_i =  \min_{u_i} \left \{ \Theta(x_N) + \sum_{i=0}^{N-1} f_i(x_i,u_i,i)     \right\}
%       \label{eq:problem_statement_reformulated}
%   \end{equation}
% subject to
% \begin{equation}
%     x_{i+1} = A_i x_i + B_i u_i, \quad x(0) =x_0
%     \label{eq:dynamic_eq_reformulated}
% \end{equation}
% \begin{equation}
%     D_i x_i + E_i u_i \leq e_i
%     \label{eq:constraint_1_reformulated}
% \end{equation}
% \begin{equation}
%      \underline{d}_i< x_i < \bar{d}_i
%     \label{eq:constraint_2_reformulated}
% \end{equation}
% where Equation \ref{eq:dynamic_eq_reformulated} represents the dynamics of the system, Equation \ref{eq:constraint_1_reformulated} represents a state-input inequality constraint and Equation \ref{eq:constraint_2_reformulated} is a pure state constraint (e.g joint limits). 

\subsubsection{Optimal framework formulation}
Following work done in \cite{li2004iterative}, \cite{murray1984differential} and \cite{del2014prioritized}, the Newton's method for nonlinear minimization is used to reformulate the optimal formulation presented in Equation (\ref{eq:problem_statement}). 
%Starting from an initial solution, linear approximations of the current dynamic model, cost function and priority constraints are defined
A new linear-quadratic constrained problem that describes the effects of perturbations on the state variables (joint positions) and input variables (joint velocities) is defined, allowing an iterative formulation of the initial optimization problem. The displacement from the measured state, $\Delta x_i = x_i - \hat{x}_{i,{des}}$ and from the input state $\Delta u_i = u_i - \hat{u}_{i,{des}}$ are expressed based on the estimated desired joint positions and velocities in Equation~(\ref{eq:estimated_path}).
% \begin{equation}
%     \Delta x_i = x_i - \hat{x}_{i_{des}}
%     \label{eq:delta_xi}
% \end{equation}
% %
% \begin{equation}
%     \Delta u_i = u_i - \hat{u}_{i_{des}}
%     \label{eq:delta_ui}
% \end{equation}
%
Using these displacements, the inequality constraints presented in Equations~(\ref{eq:joint_limits_min})-(\ref{eq:joint_limits_max}), the optimal control problem expressed by Equations~ (\ref{eq:problem_statement})-(\ref{eq:constraint_2}) can now be reformulated dependent on the state and input deviations as a linear quadratic control problem:
 \begin{equation}
 \begin{aligned}
    \Delta u^{*}_i =  \min_{\Delta u_i} &\lbrace  o_N + \Delta x_N^T q_N + \frac{1}{2} \Delta x_N^T Q_N + \Delta x_N  + \\
    & + \sum_{i=0}^{N-1} o_i + \Delta x_i q_i + \Delta u_i^T r_i + \frac{1}{2} \Delta x_i^T Q_i \Delta x_i +  \\
    & + \frac{1}{2} \Delta u_i^T R_i \Delta u_i + \Delta u_i^T P_i \Delta x_i  \rbrace
\end{aligned}
      \label{eq:problem_statement_final}
  \end{equation}
  subject to:
 \begin{equation}
    \Delta x_{i+1} = A_i \Delta x_i + B_i \Delta u_i, \quad x(0) =x_0
    \label{eq:dynamic_eq_final}
\end{equation}
\begin{equation}
    D_i \Delta x_i  = e_i %+ E_i \Delta u_i
    \label{eq:constraint_1_final}
\end{equation}
\begin{equation}
    C_i \Delta x_i = d_i
    \label{eq:constraint_2_final}
\end{equation}
% \begin{equation}
%     F_i \Delta x_i = g_i
%     \label{eq:constraint_3_final}
% \end{equation}
where $o, \ q, \ r, \ Q, \ R, \ P $ are coefficients of the Taylor expansion of Equation (\ref{eq:problem_statement}) around the estimated states. 
The linearized dynamics are presented in Equation (\ref{eq:dynamic_eq_final}) and the inequality constraints are re-defined using the potential fields in  Equations (\ref{eq:constraint_1_final}) - (\ref{eq:constraint_2_final}). To handle any possible discontinuities in the formulation of the constraints we used the method presented in \cite{stella2016very}. %\Ram{you are taylor expanding a potentially discontinuous function? That seems problematic.}. 
%
The goal is to solve this local-optimal control law generating a planning policy update, $\Delta u_i(x_i)$, which will be used in the global formulation:
\begin{equation}
    u_i(x_i) = u_i(x_i) + \Delta u_i(x_i)
    \label{eq:final_ctrl_law}
\end{equation}
This planning policy update is responsible in refining the initial planning strategy defined by Equation~(\ref{eq:estimated_path}), taking into account restrictions caused by the working environment and generating an optimal trajectory.  

Following the work of \citet{giftthaler2017projection}, we use the nullspace projection theory to present a solution for the optimal formulation in Equation (\ref{eq:problem_statement_final}), by:
\begin{equation}
   \Delta u_i = \Delta u_i^c + \mathcal{N}\left( \begin{bmatrix}
    E_i\\
    M_i
    \end{bmatrix} \right) \Delta u_i^m
    \label{eq:null_space_reform}
\end{equation}
where $\Delta u_i^c$ is the constrained  control component that ensures the constraints are always fulfilled, $E_i = D_{i+1}B_i$ and $M_i = C_{i+1} B_i$ are the propagation of the input displacements to the next step of the constraints and $\mathcal{N}$ is the projection of the nullspace of these linearized constraints. $\Delta u_i^m$ is the control component that will ensure a valid solution to the optimal problem without breaking the constraints.

The constrained control law, $\Delta u_{i}^c$, is defined to satisfy the dynamics of the constraints at the next step in time. To achieve this we propose the use of feedforward-feedback strategy:
\begin{equation}
     \Delta u_{i}^c =  \begin{bmatrix}
    E_i\\
    M_i
    \end{bmatrix}^{\dagger} 
      \begin{bmatrix}
    e_{i+1}\\
    d_{i+1}
    \end{bmatrix} -  \begin{bmatrix}
    E_i\\
    M_i
    \end{bmatrix}^{\dagger}  \begin{bmatrix}
    F_i\\
    N_i
    \end{bmatrix} (\Delta x_{i_{des}} + \alpha)
    \label{eq:feed_forward}
\end{equation}
where $ \left[ E_i^T, \ M_i^T \right]^{\dagger} $ is the unweighted Moore-Penrose pseudoinverse matrix. $F_i = D_{i+1}B_i$ and $N_i = C_{i+1}B_i$ are the propagation of the state displacements to the next step of the constraints. To compensate for the disturbances in the actuators and inaccuracies in the robot unmodeled dynamics (damping and friction), we propose to introduce a feedback law, $\alpha \in \mathbb{R}^6$,  to make the control scheme robust. The proposed feedback law is of the same type as the one presented in Section \ref{sub:lla_control}, in this case being directly dependent of the difference between the estimated state, $x_{i_{des}}$ and the measured joint positions, $x_i$. 

% \begin{figure*}[!htb]
%   \centering
%     \begin{subfigure}[]{0.32\textwidth}
%      \includegraphics[width=\textwidth]{figures/x_pos_ee_v3.png}
%      \caption{X end-effector position}
%      \label{fig:joint_2}
%      \end{subfigure}
%     \begin{subfigure}[]{0.32\textwidth}
%      \includegraphics[width=\textwidth]{figures/y_pos_ee_v3.png}
%      \caption{Y end-effector position}
%      \label{fig:x_pos}
%      \end{subfigure}
%      \begin{subfigure}[]{0.32\textwidth}
%      \includegraphics[width=\textwidth]{figures/z_pos_ee_v3.png}
%      \caption{Z end-effector position}
%      \label{fig:y_pos}
%      \end{subfigure}
%      \caption{Comparison of end-effector behavior using Optimal-Adaptive method, Adaptive strategy, \ac{RRT} and \ac{EST} methods to reach a discrete point defined in world coordinates at $(0.81, -0.05, 0.8)$ meters.  The \ac{RRT} and \ac{EST} methods require more than $4$ seconds to compute a plan but have a very fast execution, while for the Adaptive and Optimal-Adaptive methods the execution of the plan starts as soon as the first waypoint is generated, leading to a slower but more gradual movement.}
%      \label{fig:ee_x_y_z}
% \end{figure*}

\begin{figure*}[!htb]
    \centering
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[trim=10 0 30 0,clip,width=\textwidth]{figures/ee_x_lqr.png}
        \caption{X end-effector position}
        \label{fig:x_pos}
    \end{subfigure}
    ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
      %(or a blank line to force the subfigure onto a new line)
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[trim=10 10 10 10,clip,width=\textwidth]{figures/ee_y_lqr.png}
        \caption{Y end-effector position}
        \label{fig:y_pos}
    \end{subfigure}
    ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
    %(or a blank line to force the subfigure onto a new line)
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[trim=10 10 10 0,clip,width=\textwidth]{figures/ee_z_lqr.png}
        \caption{Z end-effector position}
        \label{fig:z_pos}
    \end{subfigure}
    \caption{\small{Comparison of end-effector behavior using Optimal-Adaptive method, Optimal-LQR method, Adaptive strategy, \ac{RRT} and \ac{EST} methods to reach a discrete point defined in world coordinates at $(0.81, -0.05, 0.8)$ meters.  The \ac{RRT} and \ac{EST} methods require more than $4$ seconds to compute a plan but have a very fast execution, while for the Adapt and Optimal-Adapt methods the execution of the plan starts as soon as the first waypoint is generated, leading to a slower but more gradual movement. Using the Optimal-LQR method presents a higher variation from the set-point, showcasing the limitation of an inaccurate initial guess.}}\label{fig:ee_x_y_z}
\end{figure*}


\begin{figure*}[!htb]
  \centering
    \begin{subfigure}[]{\columnwidth}
    \centering
     \includegraphics[width=0.75\columnwidth]{figures/joint_error_adapt_v2.png}
     \caption{Adaptive joint errors}
     \label{fig:error_adapt}
     \end{subfigure}
 \begin{subfigure}[]{\columnwidth}
    \centering
     \includegraphics[width=0.75\columnwidth]{figures/joint_error_optimal_v2.png}
     \caption{Optimal-Adaptive joint errors}
     \label{fig:error_optim}
     \end{subfigure}
     \caption{\small{Joint angle errors for the (a) initial Adaptive strategy and the (b) Optimal-Adaptive method when the end-effector behaviour is the one presented in Figure~\ref{fig:ee_x_y_z}. The Optimal-Adaptive strategy reduces significantly the time needed for the joints to reach the desired configuration compared with the initial Adaptive strategy, where also Joint $5$ is not able to reach the desired configuration, leading to an offset from the goal.}}
     \label{fig:joint_traj}
\end{figure*}


 
Incorporating Equations~(\ref{eq:null_space_reform})-(\ref{eq:feed_forward}) into the optimal formulation expressed by Equation (\ref{eq:problem_statement_final}), the optimal path that does not violate the constraints of the problem is defined as the solution of:
%
\begin{equation}
 \begin{aligned}
    \Delta u^{m*}_i =  \min_{\Delta u_i^m} &\lbrace  o_N + \Delta x_N^T q_N + \frac{1}{2} \Delta x_N^T Q_N + \Delta x_N  + \\
    & + \sum_{i=0}^{N-1} \tilde{o}_i + \Delta x_i \tilde{q}_i + \Delta {u_i^m}^T \tilde{r}_i + \frac{1}{2} \Delta x_i^T \tilde{Q}_i \Delta x_i +  \\
    & + \frac{1}{2} \Delta {u_i^m}^T \tilde{R}_i \Delta u_i^m + \Delta {u_i^m}^T \tilde{P}_i \Delta x_i  \rbrace
\end{aligned}
      \label{eq:problem_statement_reformulated_u}
  \end{equation}
  subject to
  \begin{equation}
    \Delta x_{i+1} = \tilde{A}_i \Delta x_i + \tilde{B}_i \Delta u_i^m + \tilde{k}_i, \quad x(0) =x_0
    \label{eq:dynamic_eq_reformulated_u}
\end{equation}
where
\begin{equation}
    \begin{aligned}
   \tilde{A}_i & = A_i + B_i \Gamma_i  \\
    %
    \tilde{B}_i & = B_i \mathcal{N(\cdot)} \\
    %
    \tilde{g}_i & = B_i \Theta_i \\
    %
    \tilde{o}_i & = o_i +  \Theta_i^T r_i + \frac{1}{2} \Theta_i^T R_i \Theta_i \\
    %
    \tilde{q}_i & = q_i + \Gamma^T r_i + P_i^T \Theta_i + \Gamma_i^TR_i \Theta_i \\
    %
    \tilde{r} & = \mathcal{N}(\cdot) \left(r_i + R_i \Gamma_i \right) \\
    %
    \tilde{Q}_i & = Q_i + \Gamma_i^T R_i \Gamma_i + \Gamma_i^T P_i + P_i^T \Gamma_i \\
    %
    \tilde{R}_i & = \mathcal{N}(\cdot) R_i \mathcal{N}(\cdot) \\
    %
    \tilde{P}_i & = \mathcal{N}(\cdot) \left(P_i + R_i \Gamma_i \right)
    \end{aligned}
    \label{eq:reparametrization}
\end{equation}

The solution of this optimal structure is computed using a Riccati equation formulation \cite{kuvcera1972discrete}, producing a feedback law presented in Equation (\ref{eq:optimal_ctrl_output}). 
\begin{equation}
\begin{aligned}
     \Delta u_i^m & = -\left( \tilde{R}_i + \tilde{B}_i^TS_{i+1}\tilde{B}_i\right)^{\dagger} \lbrace (\tilde{P}_i + \tilde{B}_i^TS_{i+1}\tilde{A}_i) \Delta x_i - \\
     & -\left[\tilde{r}_i + \tilde{B}_i^T(s_{i+1}+S_{i+1} k_i)\right] \rbrace
\end{aligned}
    \label{eq:optimal_ctrl_output}
\end{equation}
where $S_{i+1} \in \mathbb{R}^{n \times n}$ and $s_{i+1} \in \mathbb{R}^{n}$ are weighting matrices. 

The computational cost of the final planning solution, Equation (\ref{eq:final_ctrl_solution}), allows for  real-time implementation of this strategy on high-dimensional robotic systems, ensures the constraints of the problem are fulfilled and generates plans that can be fulfilled by the low-level controller. 
\begin{equation}
    \hat{u}_{i} = \hat{u}_{i_{des}} + \Delta u_i^c + \mathcal{N}(\cdot) \Delta u_i^m
    \label{eq:final_ctrl_solution}
\end{equation}

\begin{figure*}[!htb]
  \centering
    \begin{subfigure}[]{0.32\textwidth}
        \includegraphics[trim=10 0 10 0,clip, width=\textwidth]{figures/error_ee_x_lqr.png}
         \caption{Error in X}
         \label{fig:err_x_lqr}
     \end{subfigure}
     ~
    \begin{subfigure}[]{0.32\textwidth}
        \includegraphics[trim=10 0 10 0,clip, width=\textwidth]{figures/error_ee_y_lqr.png}
        \caption{Error in Y}
        \label{fig:err_y_lqr}
    \end{subfigure}
    ~
    \begin{subfigure}[]{0.32\textwidth}
        \includegraphics[trim=10 0 10 0,clip, width=\textwidth]{figures/error_ee_z_lqr.png}
        \caption{Error in Z}
        \label{fig:err_z_lqr}
    \end{subfigure}
    \caption{\small{End-effector error for the case when the joint limit presented in Figure~\ref{fig:joint_restricted} is imposed: the Optimal-Adapt (proposed) strategy reaches the vicinity of the goal fulfilling the constraints of the problem while the Optimal-LQR has a higher end-effector error, highlighting the importance of a reliable initial estimate. The \ac{RRT} method presents better accuracy  compared with any other method, nevertheless the constraints are broken and the \ac{EST} breaks the limits and also has a worse end-effector error.}}
     \label{fig:errors_ee}
\end{figure*}
%
\begin{figure}[!htb]
  \centering
    \includegraphics[width=0.85\columnwidth]{figures/joint1_limit_lqr.png}
     \caption{\small{Behaviour of Joint $1$ for the case when it can move only between ($-0.1$, $0.1$) radians. The proposed optimal strategy (Optimal-Adapt) succeeds in maintaining the joint between the boundaries (in the shaded area of the graph) as well as the Optimal-LQR method, as they both rely on the same priority-optimal principle that handles constraints.}}
     \label{fig:joint_restricted}
\end{figure}
% %
% We start our approach by defining the null-space of the linearized constraints. 
% Incorporating the system dynamics of Equation (\ref{eq:dynamic_eq_final}) into the current state constrain of Equation (\ref{eq:constraint_2_final}), the latter can be reformulated as a state-input constraint.
% %
% %To achieve this the state constrain in Equation (\ref{eq:constraint_2_final}) it is redefined in terms of state-input constraints. Using the   the state constraints at the next step can be expressed as:
% \begin{equation}
%     C_{i+1} A_i \Delta x_i + C_{i+1} B_i \Delta u_i = d_{i+1}
%     \label{eq:const_future}
% \end{equation}
% Joining together Equation (\ref{eq:constraint_1_final}) and Equation (\ref{eq:const_future}), a state-input representation of the constraint rules is expressed as:
% \begin{equation}
%     \begin{bmatrix}
%     D_i\\
%     N_i
%     \end{bmatrix} \Delta x_i +  
%      \begin{bmatrix}
%     E_i\\
%     M_i
%     \end{bmatrix} \Delta u_i =
%      \begin{bmatrix}
%     e_i\\
%     d_{i+1}
%     \end{bmatrix}
%     \label{eq:state_constraint}
% \end{equation}
% where $N_i = C_{i+1}A_i$ and $M_i = C_{i+1} B_i$ are the propagation of the state and input displacement to the next step of the constraints. The control input has to be defined to ensure a solution to the minimization  Equation (\ref{eq:problem_statement_final}) without breaking Equation (\ref{eq:state_constraint}).  According to the nullspace projection theory \cite{khatib1987unified}, a control law that satisfies Equation (\ref{eq:state_constraint}) can be defined in the form of:
% \begin{equation}
%   \Delta u_i = \Delta u_i^c + \mathcal{N}\left( \begin{bmatrix}
%     E_i\\
%     M_i
%     \end{bmatrix} \right) \Delta u_i^m
%     \label{eq:null_space_reform}
% \end{equation}
% where $\Delta u_i^c$ is the constrained  control component that ensures Equation (\ref{eq:state_constraint}) is not broken, which is going to be computed in Section \ref{sec:constrained_control_component}.  $\Delta u_i^m$ is the control component that will ensure a valid solution to the optimal problem without breaking the constraints, described in Section \ref{sec:mimim_solution}. 

%component minimizing Equation (\ref{eq:problem_statement_final}) taking into account that it can act only onto $\mathcal{N}(\cdot)$, the projected nullspace of $\left[ E_i^T \ M_i^T \right]^T$.

% \subsection{Constrained control component}
% \label{sec:constrained_control_component}
% From Equation (\ref{eq:state_constraint}), it can be seen that by applying the feedforward input in nominal conditions, a control law is generated that yields the desired behavior:
% \begin{equation}
%      \Delta u_{i_{des}}^c =  \begin{bmatrix}
%     E_i\\
%     M_i
%     \end{bmatrix}^{\dagger} 
%       \begin{bmatrix}
%     e_i\\
%     d_{i+1}
%     \end{bmatrix} -  \begin{bmatrix}
%     E_i\\
%     M_i
%     \end{bmatrix}^{\dagger}  \begin{bmatrix}
%     D_i\\
%     N_i
%     \end{bmatrix} \Delta x_{i_{des}}
%     \label{eq:feed_forward}
% \end{equation}
% where $ \begin{bmatrix} E_i\\  M_i  \end{bmatrix}^{\dagger} $ is the unweighted Moore-Penrose pseudoinverse matrix. To compensate for the disturbances in the actuators and inaccuracies in the robot unmodeled dynamics (damping and friction), feedback is introduced to make the control scheme robust. At each step, the feedback control law, Equation (\ref{eq:feed_forward_adaptive_pid}), is computed based on the state displacement error, $e_{{\Delta x}_i}  = \Delta x_{i_{des}} - \Delta x_i$, and an adaptive gain parameter, $\gamma$. This control law is powerful due to its capability to adapt to the current state of the system, removing oscillations, providing a robust response and having a small convergence time.
% %
% \begin{equation}
%     \alpha_i =  \gamma  e_{{\Delta x}_i} \left[ e_{{\Delta x}_i} \mid  e_{{\Delta x}_i} \mid +  \dot{e}_{{\Delta x}_i}^2  +   \left( \sum_{j=0}^i  e_{{\Delta x}_j} \tau \right)^2 \right]
%     \label{eq:feed_forward_adaptive_pid}
% \end{equation}
% Introducing Equation (\ref{eq:feed_forward_adaptive_pid}) in Equation (\ref{eq:feed_forward}), the control law for $\Delta u_i^c$ is computed by:
% \begin{equation}
%      \Delta u_{i}^c =  \begin{bmatrix}
%     E_i\\
%     M_i
%     \end{bmatrix}^{\dagger} 
%       \begin{bmatrix}
%     e_i\\
%     d_{i+1}
%     \end{bmatrix} -  \begin{bmatrix}
%     E_i\\
%     M_i
%     \end{bmatrix}^{\dagger}  \begin{bmatrix}
%     D_i\\
%     N_i
%     \end{bmatrix} \left( \Delta x_{i_{des}} + \alpha \right)
%     \label{eq:feed_forward_adaptive}
% \end{equation}
% This control law ensures that the constraints are not violated while not allowing the state displacement to deviate from the control nullspace. 

% % Replacing Equation (\ref{eq:feed_forward_adaptive}) in Equation (\ref{eq:null_space_reform}) we obtain:
% % \begin{equation}
% % \begin{aligned}
% %   \Delta u_i = \begin{bmatrix}
% %     E_i\\
% %     M_i
% %     \end{bmatrix}^{\dagger} 
% %       \begin{bmatrix}
% %     e_i\\
% %     d_{i+1}
% %     \end{bmatrix} -  \begin{bmatrix}
% %     E_i\\
% %     M_i
% %     \end{bmatrix}^{\dagger}  \begin{bmatrix}
% %     D_i\\
% %     N_i
% %     \end{bmatrix} \left( \Delta x_{i_{des}} + \alpha \right) + \mathcal{N}\left( \begin{bmatrix}
% %     E_i\\
% %     M_i
% %     \end{bmatrix} \right) \Delta u_i^m
% % \end{aligned}
% %     \label{eq:null_space_updated}
% % \end{equation}
% Replacing Equation (\ref{eq:feed_forward_adaptive}) in Equation (\ref{eq:null_space_reform}),  we obtain: 
% \begin{equation}
%     \Delta u _i = \Theta_i - \Gamma_i \Delta x_i + \mathcal{N}(\cdot) \Delta u_i^m
%     \label{eq:u_i_const}
% \end{equation}
% where:
% \begin{equation}
% \begin{aligned}
%     \kappa & = \begin{bmatrix}
%     E_i\\
%     M_i
%     \end{bmatrix}^{\dagger} 
%       \begin{bmatrix}
%     e_i\\
%     d_{i+1}
%     \end{bmatrix} \\
%     \epsilon & = \begin{bmatrix}
%     E_i\\
%     M_i
%     \end{bmatrix}^{\dagger}  \begin{bmatrix}
%     D_i\\
%     N_i
%     \end{bmatrix} \\
%     \Theta & = \kappa - \epsilon \Delta x_{i_{des}} - \epsilon \gamma \Delta x_{i_{des}} \cdot \\   
%     &\cdot  \left[ e_{{\Delta x}_i} \mid  e_{{\Delta x}_i} \mid + \dot{e}_{{\Delta x}_i}^2  +   \left( \sum_{j=0}^i  e_{{\Delta x}_j} \tau \right)^2 \right] \\
%     \Gamma & = - \epsilon \left[ e_{{\Delta x}_i} \mid  e_{{\Delta x}_i} \mid + \dot{e}_{{\Delta x}_i}^2  +   \left( \sum_{j=0}^i  e_{{\Delta x}_j} \tau \right)^2 \right]
%     \end{aligned}
%     \label{eq:notations}
% \end{equation}



% \subsection{Optimal control solution}
% \label{sec:mimim_solution}
% While the control law in Equation (\ref{eq:u_i_const}) ensures that the constraints are not violated, it also has to represent the solution to the optimal problem. To achieve this,  we reformulate the cost function in Equation (\ref{eq:problem_statement_final}), and the dynamic Equation (\ref{eq:dynamic_eq_final}) is dependent on the  input $\Delta u_i^m$:

%  \begin{equation}
%  \begin{aligned}
%     \Delta u^{m*}_i =  \min_{\Delta u_i^m} &\lbrace  o_N + \Delta x_N^T q_N + \frac{1}{2} \Delta x_N^T Q_N + \Delta x_N  + \\
%     & + \sum_{i=0}^{N-1} \tilde{o}_i + \Delta x_i \tilde{q}_i + \Delta {u_i^m}^T \tilde{r}_i + \frac{1}{2} \Delta x_i^T \tilde{Q}_i \Delta x_i +  \\
%     & + \frac{1}{2} \Delta {u_i^m}^T \tilde{R}_i \Delta u_i^m + \Delta {u_i^m}^T \tilde{P}_i \Delta x_i  \rbrace
% \end{aligned}
%       \label{eq:problem_statement_reformulated_u}
%   \end{equation}
%   subject to
%   \begin{equation}
%     \Delta x_{i+1} = \tilde{A}_i \Delta x_i + \tilde{B}_i \Delta u_i^m + \tilde{k}_i, \quad x(0) =x_0
%     \label{eq:dynamic_eq_reformulated_u}
% \end{equation}
% where
% \begin{equation}
%     \begin{aligned}
%   \tilde{A}_i & = A_i + B_i \Gamma_i  \\
%     %
%     \tilde{B}_i & = B_i \mathcal{N(\cdot)} \\
%     %
%     \tilde{g}_i & = B_i \Theta_i \\
%     %
%     \tilde{o}_i & = o_i +  \Theta_i^T r_i + \frac{1}{2} \Theta_i^T R_i \Theta_i \\
%     %
%     \tilde{q}_i & = q_i + \Gamma^T r_i + P_i^T \Theta_i + \Gamma_i^TR_i \Theta_i \\
%     %
%     \tilde{r} & = \mathcal{N}(\cdot) \left(r_i + R_i \Gamma_i \right) \\
%     %
%     \tilde{Q}_i & = Q_i + \Gamma_i^T R_i \Gamma_i + \Gamma_i^T P_i + P_i^T \Gamma_i \\
%     %
%     \tilde{R}_i & = \mathcal{N}(\cdot) R_i \mathcal{N}(\cdot) \\
%     %
%     \tilde{P}_i & = \mathcal{N}(\cdot) \left(P_i + R_i \Gamma_i \right)
%     \end{aligned}
%     \label{eq:reparametrization}
% \end{equation}

% For this problem, the Lagrange multiplyer method is applied to compute the control input, and the problem is being formulated with a \ac{LQ} structure. Considering the Hamiltonian quantity in Equation (\ref{eq:hamilton}), the optimal control input is defined using its derivative with respect to the control input, as presented in Equation (\ref{eq:detiv_ctrl}).
% \begin{equation}
% \begin{aligned}
%      \mathcal{L}(\Delta x_i, \delta u_i, \lambda) & = \tilde{o}_i + \Delta x_i \tilde{q}_i + \Delta {u_i^m}^T \tilde{r}_i + \frac{1}{2} \Delta x_i^T \tilde{Q}_i \Delta x_i +  \\
%     & + \frac{1}{2} \Delta {u_i^m}^T \tilde{R}_i \Delta u_i^m + \Delta {u_i^m}^T \tilde{P}_i \Delta x_i + \\
%     & +\lambda^T \left( \tilde{A}_i \Delta x_i + \tilde{B}_i \Delta u_i^m + \tilde{k}_i \right)
% \end{aligned}
%     \label{eq:hamilton}
% \end{equation}
% %
% \begin{equation}
%   \begin{aligned}
%     \frac{d\mathcal{L}}{d \Delta u_i^m} & = \tilde{r}_i + \tilde{R}_i \delta u_i^m + \tilde{P}_i \Delta x_i + \lambda^T B_i = 0 \\
%     \Rightarrow \Delta u_i^m & = -\tilde{R}_i^{\dagger} \left[ \tilde{r}_i + \tilde{P}_i \Delta x_i + \lambda^T \tilde{B}_i \right]
%     \end{aligned}
%     \label{eq:detiv_ctrl}
% \end{equation}
% where $\tilde{R}_i^{\dagger}$ is the unweighted Moore-Penrose pseudoinverse. Incorporating Equation (\ref{eq:detiv_ctrl}) into the Hamiltonian quantity Equation (\ref{eq:hamilton}), the optimized Hamiltonian quantity is obtained:
% \begin{equation}
% \begin{aligned}
%     & \mathcal{L}^{*}(\Delta x_i, \lambda)  = \tilde{o}_i + \Delta x_i \tilde{q}_i - \left[ \tilde{r}_i^T +  \Delta x_i^T \tilde{P}_i^T + \tilde{B}_i^T \lambda \right] \tilde{R}_i^{\dagger T} \tilde{r}_i + \\ 
%     & +\frac{1}{2} \Delta x_i^T \tilde{Q}_i \Delta x_i - \left[ \tilde{r}_i^T +  \Delta x_i^T \tilde{P}_i^T + \tilde{B}_i^T \lambda \right] \tilde{R}_i^{\dagger T} \tilde{P}_i \Delta x_i + \\
%     & + \frac{1}{2} \left[ \tilde{r}_i^T +  \Delta x_i^T \tilde{P}_i^T + \tilde{B}_i^T \lambda \right] \tilde{R}_i^{\dagger T} \tilde{R}_i \tilde{R}_i^{\dagger} \left[ \tilde{r}_i + \tilde{P}_i \Delta x_i + \lambda^T \tilde{B}_i \right] + \\
%     & +\lambda^T \lbrace \tilde{A}_i \Delta x_i - \tilde{B}_i \tilde{R}_i^{\dagger} \left[ \tilde{r}_i + \tilde{P}_i \Delta x_i + \lambda^T \tilde{B}_i \right]+ \tilde{k}_i \rbrace = 0
%     \end{aligned}
% \end{equation}
% By doing a sweep method such as $\lambda = \Delta x_i^T s_i + \frac{1}{2} \Delta x_i^T S_i \Delta x_i$ the following Riccati equation is obtained:
% \begin{equation}
% \begin{aligned}
%     & - (\tilde{P}_i +\tilde{A}_i^TS_i \tilde{B}_i)(\tilde{R}_i + \tilde{B}_i^TS_i\tilde{B}_i)^{-1}(\tilde{P}_i+\tilde{B}_i^TS_i\tilde{A}_i)  - \\
%     & -\left[ r_i + (s_i+S_i)k_i \tilde{B}_i\right] (\tilde{R}_i + \tilde{B}_i^T S_i \tilde{B}_i)^{-1} \left[r_i + \tilde{B}_i^T k_i (s_i + S_i) \right] + \\
%     & + \tilde{A}_i^T S_i \tilde{A}_i + \tilde{Q}= 0
% \end{aligned}
%     \label{eq:riccati_equation}
% \end{equation}
% where $s_i \in \mathbb{R}^n$ and $S_i \in \mathbb{R}^{n \times n}$ are the weighting matrices. 
% From this formulation, the optimal control formulation can be defined as:
% \begin{equation}
% \begin{aligned}
%      \Delta u_i^m & = -\left( \tilde{R}_i + \tilde{B}_i^TS_{i+1}\tilde{B}_i\right)^{\dagger} \lbrace (\tilde{P}_i + \tilde{B}_i^TS_{i+1}\tilde{A}_i) \Delta x_i - \\
%      & -\left[\tilde{r}_i + \tilde{B}_i^T(s_{i+1}+S_{i+1} k_i)\right] \rbrace
% \end{aligned}
%     \label{eq:optimal_ctrl_output}
% \end{equation}
% Incorporating Equation (\ref{eq:null_space_reform}) and Equation (\ref{eq:optimal_ctrl_output}), the control feedback law is:
% \begin{equation}
% \begin{aligned}
%     u_i & = u_i + \Theta_i - \Gamma_i \left( \tilde{R}_i + \tilde{B}_i^TS_{i+1}\tilde{B}_i\right)^{\dagger} \cdot \\ 
%     & \cdot \lbrace (\tilde{P}_i + \tilde{B}_i^TS_{i+1}\tilde{A}_i) \Delta x_i  -\left[\tilde{r}_i + \tilde{B}_i^T(s_{i+1}+S_{i+1} k_i)\right] \rbrace
% \end{aligned}
%     \label{eq:final_ctrl_law}
% \end{equation}


% % This section presents a method for computing the control increments $\Delta u^*$. The proposed algorithm is based on the nullspace projection theory \cite{khatib1987unified} to ensure the constraints are fulfilled, and it uses a Riccati equation formulation \cite{kuvcera1972discrete} to compute the feedback law. 

% % To define the local control problem, a stable initial control policy $u_{0} \in \mathbb{R}^m$ is needed. We will use an adaptive control law that requires minimum tuning and ensures stable behavior of the system. This control law will be presented extensively in Section \ref{sec:proposed_method}.  Starting from this initial control output and the initial conditions  $x_0 \in \mathbb{R}^n$, in each iteration the estimated state $\hat{x}_i$ is computed using the dynamic equation, and the estimated control  input $\hat{u}_i$ is determined using the current control policy. 

% %A detailed description of the mapping of Equations \ref{eq:problem_statement} - \ref{eq:constraint_2} to Equations  \ref{eq:problem_statement_final} - \ref{eq:constraint_3_final} is given in \cite{del2014prioritized}.

